Advancing SVD-based LLM Compression via Layer-Wise Error Model Search

Low-rank SVD-based compression offers a powerful strategy to reduce the computational costs of LLMs. However, existing methods face two key limitations: (i) global rank allocation, where uncalibrated error proxies fail to capture complex error propagation, and (ii) decomposition quality, where Fisher-based estimators suffer from severe rank collapse. In this work, we address these limitations by introducing Layer-wise Error Modeling Search (LEMS) and KFAC-SVD. LEMS advances rank allocation by introducing a layer-wise error surrogate that integrates local and global layer importance alongside a propagation bias, enabling effective global rank allocation via an ILP formulation. KFAC-SVD improves decomposition quality by utilizing token-wise statistics, mitigating the rank deficiency observed in prior Fisher-based SVD approaches. Across Mistral, Qwen3, and Llama 3 model families, we show that LEMS consistently outperforms existing search strategies, delivering significant zero-shot accuracy gains of up to 4.7 p.p. that generalize to model sizes of 70B parameters, while KFAC-SVD achieves an average perplexity improvement of 19%. Project page and code: https://lems-svd.github.io

==> main.gls.tex <==
\glossarysection[\glossarytoctitle]{\glossarytitle}\glossarypreamble
\begin{theglossary}\glossaryheader
\glsgroupheading{A}\relax \glsresetentrylist %
\glossentry{ars}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{2}\delimN 
		\setentrycounter[]{page}\glsnumberformat{5\delimN 6}\delimN 
		\setentrycounter[]{page}\glsnumberformat{14}\delimN 
		\setentrycounter[]{page}\glsnumberformat{23}\delimN 
		\setentrycounter[]{page}\glsnumberformat{35\delimN 36}}}%
\glossentry{asvd}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{2}\delimN 
		\setentrycounter[]{page}\glsnumberformat{5\delimR 7}\delimN 
		\setentrycounter[]{page}\glsnumberformat{14\delimN 15}\delimN 
		\setentrycounter[]{page}\glsnumberformat{17\delimR 25}\delimN 
		\setentrycounter[]{page}\glsnumberformat{29}\delimN 
		\setentrycounter[]{page}\glsnumberformat{34\delimR 36}}}%
\glossentry{atp}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{3}\delimN 
		\setentrycounter[]{page}\glsnumberformat{5\delimN 6}\delimN 
		\setentrycounter[]{page}\glsnumberformat{14\delimN 15}\delimN 
		\setentrycounter[]{page}\glsnumberformat{18}\delimN 
		\setentrycounter[]{page}\glsnumberformat{20}\delimN 
		\setentrycounter[]{page}\glsnumberformat{23\delimR 25}\delimN 
		\setentrycounter[]{page}\glsnumberformat{35\delimN 36}}}\glsgroupskip
\glsgroupheading{B}\relax \glsresetentrylist %
\glossentry{basissharing}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{6}\delimN 
		\setentrycounter[]{page}\glsnumberformat{25\delimR 27}}}%
\glossentry{bitstack}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{2}\delimN 
		\setentrycounter[]{page}\glsnumberformat{6}\delimN 
		\setentrycounter[]{page}\glsnumberformat{25\delimN 26}}}\glsgroupskip
\glsgroupheading{C}\relax \glsresetentrylist %
\glossentry{c4}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{6\delimN 7}\delimN 
		\setentrycounter[]{page}\glsnumberformat{22\delimN 23}\delimN 
		\setentrycounter[]{page}\glsnumberformat{25}\delimN 
		\setentrycounter[]{page}\glsnumberformat{27\delimR 29}\delimN 
		\setentrycounter[]{page}\glsnumberformat{34\delimR 36}}}%
\glossentry{comcat}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{2}}}\glsgroupskip
\glsgroupheading{D}\relax \glsresetentrylist %
\glossentry{dobisvd}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{2}\delimN 
		\setentrycounter[]{page}\glsnumberformat{5\delimR 7}\delimN 
		\setentrycounter[]{page}\glsnumberformat{22}\delimN 
		\setentrycounter[]{page}\glsnumberformat{25}\delimN 
		\setentrycounter[]{page}\glsnumberformat{29}\delimN 
		\setentrycounter[]{page}\glsnumberformat{34\delimN 35}}}\glsgroupskip
\glsgroupheading{F}\relax \glsresetentrylist %
\glossentry{fastlrd}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{2}}}%
\glossentry{flarsvd}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{2}}}%
\glossentry{fwsvd}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{5}\delimN 
		\setentrycounter[]{page}\glsnumberformat{7}\delimN 
		\setentrycounter[]{page}\glsnumberformat{22}\delimN 
		\setentrycounter[]{page}\glsnumberformat{25}\delimN 
		\setentrycounter[]{page}\glsnumberformat{29}\delimN 
		\setentrycounter[]{page}\glsnumberformat{34\delimN 35}}}\glsgroupskip
\glsgroupheading{G}\relax \glsresetentrylist %
\glossentry{gfwsvd}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{2\delimR 5}\delimN 
		\setentrycounter[]{page}\glsnumberformat{7\delimN 8}\delimN 
		\setentrycounter[]{page}\glsnumberformat{21\delimN 22}\delimN 
		\setentrycounter[]{page}\glsnumberformat{25}\delimN 
		\setentrycounter[]{page}\glsnumberformat{29}\delimN 
		\setentrycounter[]{page}\glsnumberformat{34\delimN 35}}}\glsgroupskip
\glsgroupheading{I}\relax \glsresetentrylist %
\glossentry{ilp}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{1\delimR 6}\delimN 
		\setentrycounter[]{page}\glsnumberformat{8}\delimN 
		\setentrycounter[]{page}\glsnumberformat{16\delimN 17}\delimN 
		\setentrycounter[]{page}\glsnumberformat{19}\delimN 
		\setentrycounter[]{page}\glsnumberformat{27}\delimN 
		\setentrycounter[]{page}\glsnumberformat{33}}}\glsgroupskip
\glsgroupheading{K}\relax \glsresetentrylist %
\glossentry{kfac}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{8}\delimN 
		\setentrycounter[]{page}\glsnumberformat{21\delimR 23}\delimN 
		\setentrycounter[]{page}\glsnumberformat{32}}}%
\glossentry{ours}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{1\delimR 4}\delimN 
		\setentrycounter[]{page}\glsnumberformat{6\delimR 9}\delimN 
		\setentrycounter[]{page}\glsnumberformat{14}\delimN 
		\setentrycounter[]{page}\glsnumberformat{21\delimR 31}\delimN 
		\setentrycounter[]{page}\glsnumberformat{34\delimN 35}\delimN 
		\setentrycounter[]{page}\glsnumberformat{37}}}%
\glossentry{kl}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{5}\delimN 
		\setentrycounter[]{page}\glsnumberformat{8}\delimN 
		\setentrycounter[]{page}\glsnumberformat{14}\delimN 
		\setentrycounter[]{page}\glsnumberformat{16\delimR 21}\delimN 
		\setentrycounter[]{page}\glsnumberformat{23}\delimN 
		\setentrycounter[]{page}\glsnumberformat{33}}}\glsgroupskip
\glsgroupheading{L}\relax \glsresetentrylist %
\glossentry{oursearch}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{1\delimR 9}\delimN 
		\setentrycounter[]{page}\glsnumberformat{14\delimN 15}\delimN 
		\setentrycounter[]{page}\glsnumberformat{18\delimR 20}\delimN 
		\setentrycounter[]{page}\glsnumberformat{22\delimR 25}\delimN 
		\setentrycounter[]{page}\glsnumberformat{27\delimR 29}\delimN 
		\setentrycounter[]{page}\glsnumberformat{31}\delimN 
		\setentrycounter[]{page}\glsnumberformat{33\delimR 37}}}%
\glossentry{llama}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{22\delimR 25}}}%
\glossentry{llama2}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{14}\delimN 
		\setentrycounter[]{page}\glsnumberformat{22}\delimN 
		\setentrycounter[]{page}\glsnumberformat{25}\delimN 
		\setentrycounter[]{page}\glsnumberformat{27}}}%
\glossentry{llama3}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{1\delimN 2}\delimN 
		\setentrycounter[]{page}\glsnumberformat{5\delimR 8}\delimN 
		\setentrycounter[]{page}\glsnumberformat{14\delimR 22}\delimN 
		\setentrycounter[]{page}\glsnumberformat{24\delimR 26}\delimN 
		\setentrycounter[]{page}\glsnumberformat{28\delimN 29}\delimN 
		\setentrycounter[]{page}\glsnumberformat{34\delimR 36}}}%
\glossentry{llm}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{1\delimR 3}\delimN 
		\setentrycounter[]{page}\glsnumberformat{5\delimR 7}\delimN 
		\setentrycounter[]{page}\glsnumberformat{9}\delimN 
		\setentrycounter[]{page}\glsnumberformat{14\delimN 15}\delimN 
		\setentrycounter[]{page}\glsnumberformat{29}}}\glsgroupskip
\glsgroupheading{M}\relax \glsresetentrylist %
\glossentry{mdp}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{3}}}%
\glossentry{mistral}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{1\delimN 2}\delimN 
		\setentrycounter[]{page}\glsnumberformat{5\delimR 7}\delimN 
		\setentrycounter[]{page}\glsnumberformat{14}\delimN 
		\setentrycounter[]{page}\glsnumberformat{19}\delimN 
		\setentrycounter[]{page}\glsnumberformat{21}\delimN 
		\setentrycounter[]{page}\glsnumberformat{24\delimN 25}\delimN 
		\setentrycounter[]{page}\glsnumberformat{28\delimN 29}\delimN 
		\setentrycounter[]{page}\glsnumberformat{34\delimR 36}}}%
\glossentry{mlp}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{2}\delimN 
		\setentrycounter[]{page}\glsnumberformat{4}\delimN 
		\setentrycounter[]{page}\glsnumberformat{17}}}%
\glossentry{moe}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{9}}}%
\glossentry{mrcs}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{2}\delimN 
		\setentrycounter[]{page}\glsnumberformat{5\delimN 6}\delimN 
		\setentrycounter[]{page}\glsnumberformat{14}\delimN 
		\setentrycounter[]{page}\glsnumberformat{17}\delimN 
		\setentrycounter[]{page}\glsnumberformat{19\delimR 21}\delimN 
		\setentrycounter[]{page}\glsnumberformat{23\delimR 25}\delimN 
		\setentrycounter[]{page}\glsnumberformat{35\delimN 36}}}%
\glossentry{mse}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{8}\delimN 
		\setentrycounter[]{page}\glsnumberformat{18}}}\glsgroupskip
\glsgroupheading{P}\relax \glsresetentrylist %
\glossentry{pp}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{1\delimN 2}\delimN 
		\setentrycounter[]{page}\glsnumberformat{6\delimR 8}\delimN 
		\setentrycounter[]{page}\glsnumberformat{24}\delimN 
		\setentrycounter[]{page}\glsnumberformat{27\delimN 28}}}%
\glossentry{ptb}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{6\delimN 7}\delimN 
		\setentrycounter[]{page}\glsnumberformat{22\delimN 23}\delimN 
		\setentrycounter[]{page}\glsnumberformat{25}\delimN 
		\setentrycounter[]{page}\glsnumberformat{27\delimR 29}\delimN 
		\setentrycounter[]{page}\glsnumberformat{34\delimR 36}}}\glsgroupskip
\glsgroupheading{Q}\relax \glsresetentrylist %
\glossentry{qwen3}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{1\delimN 2}\delimN 
		\setentrycounter[]{page}\glsnumberformat{5\delimR 8}\delimN 
		\setentrycounter[]{page}\glsnumberformat{14\delimR 22}\delimN 
		\setentrycounter[]{page}\glsnumberformat{24\delimN 25}\delimN 
		\setentrycounter[]{page}\glsnumberformat{28\delimR 30}\delimN 
		\setentrycounter[]{page}\glsnumberformat{34\delimR 37}}}\glsgroupskip
\glsgroupheading{S}\relax \glsresetentrylist %
\glossentry{svd}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{1\delimR 9}\delimN 
		\setentrycounter[]{page}\glsnumberformat{14}\delimN 
		\setentrycounter[]{page}\glsnumberformat{21\delimR 23}\delimN 
		\setentrycounter[]{page}\glsnumberformat{25\delimR 29}\delimN 
		\setentrycounter[]{page}\glsnumberformat{31\delimN 32}\delimN 
		\setentrycounter[]{page}\glsnumberformat{34}}}%
\glossentry{svdllm}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{2\delimN 3}\delimN 
		\setentrycounter[]{page}\glsnumberformat{5}\delimN 
		\setentrycounter[]{page}\glsnumberformat{7\delimN 8}\delimN 
		\setentrycounter[]{page}\glsnumberformat{22}\delimN 
		\setentrycounter[]{page}\glsnumberformat{24\delimN 25}\delimN 
		\setentrycounter[]{page}\glsnumberformat{28\delimR 30}\delimN 
		\setentrycounter[]{page}\glsnumberformat{34\delimN 35}\delimN 
		\setentrycounter[]{page}\glsnumberformat{37}}}%
\glossentry{svdllmv2}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{2}\delimN 
		\setentrycounter[]{page}\glsnumberformat{5\delimR 7}\delimN 
		\setentrycounter[]{page}\glsnumberformat{14}\delimN 
		\setentrycounter[]{page}\glsnumberformat{17}\delimN 
		\setentrycounter[]{page}\glsnumberformat{22\delimR 25}\delimN 
		\setentrycounter[]{page}\glsnumberformat{29}\delimN 
		\setentrycounter[]{page}\glsnumberformat{34\delimR 36}}}\glsgroupskip
\glsgroupheading{T}\relax \glsresetentrylist %
\glossentry{tpe}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{5}\delimN 
		\setentrycounter[]{page}\glsnumberformat{16\delimN 17}\delimN 
		\setentrycounter[]{page}\glsnumberformat{33}}}\glsgroupskip
\glsgroupheading{V}\relax \glsresetentrylist %
\glossentry{vlm}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{9}}}\glsgroupskip
\glsgroupheading{W}\relax \glsresetentrylist %
\glossentry{wiki}{\glossaryentrynumbers{\relax 
		\setentrycounter[]{page}\glsnumberformat{2}\delimN 
		\setentrycounter[]{page}\glsnumberformat{5\delimR 8}\delimN 
		\setentrycounter[]{page}\glsnumberformat{18}\delimN 
		\setentrycounter[]{page}\glsnumberformat{21\delimR 29}\delimN 
		\setentrycounter[]{page}\glsnumberformat{34\delimR 36}}}%
\end{theglossary}\glossarypostamble

